The Evolving Usage of GenAI by Computing Students

Help-seeking is a critical aspect of learning and problem-solving for computing students. Recent research has shown that many students are aware of generative AI (GenAI) tools; however, there are gaps in the extent and effectiveness of how students use them. With over two years of widespread GenAI usage, it is crucial to understand whether students' help-seeking behaviors with these tools have evolved and how. This paper presents findings from a repeated cross-sectional survey conducted among computing students across North American universities (n=95). Our results indicate shifts in GenAI usage patterns. In 2023, 34.1% of students (n=47) reported never using ChatGPT for help, ranking it fourth after online searches, peer support, and class forums. By 2024, this figure dropped sharply to 6.3% (n=48), with ChatGPT nearly matching online search as the most commonly used help resource. Despite this growing prevalence, there has been a decline in students' hourly and daily usage of GenAI tools, which may be attributed to a common tendency to underestimate usage frequency. These findings offer new insights into the evolving role of GenAI in computing education, highlighting its increasing acceptance and solidifying its position as a key help resource.

==> 35-error-table.tex <==

\begin{table}[!h]
%  \small
  \footnotesize
  \caption{Student Mistakes from Altadmri and Brown~\cite{altadmri201537}}
  \label{tab:study-1-bug-types}
  \begin{tabular}{cl}
    
    \toprule
    \textbf{Shorthand} & \textbf{Explanation of the Mistake} \\
    \midrule
    \multicolumn{2}{l}{\textit{Syntax errors:}} \\
    A & Confusing \texttt{=} with \texttt{==} \\ % Bug Code: A
    C & Mismatched parentheses \\ % Bug Code: C
    D & Confusing \texttt{\&} with \texttt{\&\&} \\ % Bug Code: D*
    E & Spurious semi-colon after \texttt{if}, \texttt{for}, \texttt{while}\\ % Bug Code: E*
    F & Wrong separator in \texttt{for} \\% Bug Code: F
    G & Wrong brackets in \texttt{if} \\ % Bug Code: G
    H & Using reserved keywords \\ % Bug Code: H
    J & Forgetting parentheses when calling methods \\ % Bug Code: J
    K & Spurious semi-colon after method header \\ % Bug Code: K
    L & Less-than / greater-than operators wrong \\ % Bug Code: L
    P & Including types in actual method arguments\\ % Bug Code: P
    \midrule
    \multicolumn{2}{l}{\textit{Type errors:}}\\ 
    I & Calling method with wrong types \\ % Bug Code: I
    Q & Type mismatch when assigning method result \\ % Bug Code: Q
    \midrule
    \multicolumn{2}{l}{\textit{Other semantic errors:}} \\
    B & Using \texttt{==} to compare strings \\ % Bug Code: B*
    M & Invoking instance method as static \\ % Bug Code: M
    N & Discarding method return \\ % Bug Code: N*
    O & Missing return statement \\ % Bug Code: O
    R & Missing methods when implementing interface \\ % Bug Code: R
    
  \bottomrule
\end{tabular}
\end{table}

